Linear Insertion Deletion Codes in the High-Noise and High-Rate Regimes

This work continues the study of linear error correcting codes against adversarial insertion deletion errors (insdel errors). Previously, the work of Cheng, Guruswami, Haeupler, and Li \cite{CGHL21} showed the existence of asymptotically good linear insdel codes that can correct arbitrarily close to $1$ fraction of errors over some constant size alphabet, or achieve rate arbitrarily close to $1/2$ even over the binary alphabet. As shown in \cite{CGHL21}, these bounds are also the best possible. However, known explicit constructions in \cite{CGHL21}, and subsequent improved constructions by Con, Shpilka, and Tamo \cite{9770830} all fall short of meeting these bounds. Over any constant size alphabet, they can only achieve rate $< 1/8$ or correct $< 1/4$ fraction of errors; over the binary alphabet, they can only achieve rate $< 1/1216$ or correct $< 1/54$ fraction of errors. Apparently, previous techniques face inherent barriers to achieve rate better than $1/4$ or correct more than $1/2$ fraction of errors. In this work we give new constructions of such codes that meet these bounds, namely, asymptotically good linear insdel codes that can correct arbitrarily close to $1$ fraction of errors over some constant size alphabet, and binary asymptotically good linear insdel codes that can achieve rate arbitrarily close to $1/2$.\ All our constructions are efficiently encodable and decodable. Our constructions are based on a novel approach of code concatenation, which embeds the index information implicitly into codewords. This significantly differs from previous techniques and may be of independent interest. Finally, we also prove the existence of linear concatenated insdel codes with parameters that match random linear codes, and propose a conjecture about linear insdel codes.

==> construction_hrate2_backup.tex <==
\section{For Rate Close to 1/2}

In this section we modify our construction in the previous section to give a linear insdel code with rate close to $1/2$.

\begin{theorem}\label{thm:highrate2}
For every constant $\gamma \in (0, 1)$, there exists a binary linear insdel codes with rate $\ge 1/2 - \gamma$, relative decoding radius  $\rho \ge  \Omega(1)$.
\end{theorem}

\paragraph{The construction.} Following our general construction, here we take $\Cout$ to be an $[n,k,d]_{q}$ Algebraic Geometry code with $|\alphabetout| = q = O(\frac{n}{d})^2$, $k = (1- O(\delta)) n$ and $d = \delta  n$ for  $\delta = \gamma/2$. 
We construct $n$ different binary inner codes $\Cin^1, \dots, \Cin^n$, with codeword length $n'$, message length $k'= \log  q = (\frac{1}{2}-\gamma/2)n'$ such that they satisfy the following property with parameters $s = O(\log n), d' = $.

We need the following dense property.
\begin{lemma}
Let $y, y'$ be two distinct codewords of the outer code, then for every $\ell  = O(\log n)$, if we cut $y, y'$ into   non-overlapping substrings of length $\ell$, then for at least a $\frac{d}{2n}$ fraction of these substrings $y_t, t\in [\ell]$,   the distance between $y_t$ and $y'_{t}$ is at least  $ \frac{d}{2n} \ell $.
\end{lemma}
\begin{proof}
Suppose not. 
There are less than $\frac{d}{2n}$ fraction of these substrings $y_t, t\in [\ell]$,   the distance between $y_t$ and $y'_{t}$ is at least  $ \frac{d}{2n} \ell $.
Then the total distance is at most $\frac{d}{2n} \times n + (1-\frac{d}{2n}) \times n \times \frac{d}{2n} < d $, which contradicts the distance of the outer code.

\end{proof}










\begin{property}[$s, d'$]
\label{prop:propertymain-s}
$\forall t\in [n], \forall i \in [n-t], j \in [n-t-1]$, $\forall w = w_i \circ \cdots \circ w_{i-1+t} \in \bigcirc_{k\in [t]} \Cin^{i-1+k}$,  $\forall u = u_j \circ u_{j+1} \circ \cdots \circ u_{j+t}\in \bigcirc_{k\in [t+1]}\Cin^{j-1+k}$, 
it always holds that for any substring $ w' $ of $u$, we have $\ed(w, w')\ge   d'$, 
as long as the following holds
\begin{itemize}
    \item The number of non-zero blocks in $w$ and $u$ together is  $r \in [s, 10s]$.
    \item Among them there are at least $r_1 = r \gamma/2 $ blocks  such that for each one there is no block  in $u$ that is the same codeword in a same inner code. 
    Call this kind of blocks as unique blocks.
\end{itemize}

We say the property is with parameter $(s, d')$ to indicate the parameters $s, d'$.
\end{property}

Recall that we denote the concatenated code as $\C$.

\begin{lemma}
For every $s, d'\in [n], s  \ge 10/\gamma,  d' = O(n')$, there exists an efficient construction of $n$ binary codes $\Cin^1, \dots, \Cin^n$ satisfying \cref{prop:propertymain-s} with parameter $s, d'$, where each $\Cin^i$ has rate $\gamma_i =  \frac{1}{2}- \gamma/2 $.
\end{lemma}
\begin{proof}
We  show that if the basis of the $n$ linear codes are randomly generated, then with high probability, the property holds.

As there are exactly $r$ non-zero blocks in $w, u$,
the number of different positions of zero blocks in $w$ and $u$ is ${2t+1 \choose r}$.
Now fix the positions of the non-zero blocks.



Consider an arbitrary substring $w'$ of $u$.
Suppose $\ed(w, w') < d'$.
Then $\lcs(w, w') \ge (|w|+|w'| - d')/2 > |w| - d'$, since $|w'| > |w|-d$.

Let $M$ be a maximum matching between $w, w'$.
Consider any  match $(i, i)$   in $M$ such that the two blocks that they are in, are non-zero and are exactly the same.
Denote the number of such matches as $m_1$.
Remove these matches from $M$.
Next consider any match $(i, j)$ such that both $i$ and $j$ are from zero blocks.
Denote the number of such matches as $m_2$.
Also remove these matches from $M$.
Now denote the matching after these removes as $M'$.
Notice that $|M'| > |w| - m_1 - m_2-d' = tn_0 - m_1 - m_2 -d'$.
Notice that these removed matches will always be correct matches.
For each of the remaining match, the probability that it is a correct match is $1/2$, since we choose random independent basis.
The probability that all matches in $M'$  are correct is $2^{-|M'|}$.

Next we do the union bound.
Notice that the number of unique blocks in $w$ and $u$ is $r_1 \ge r \gamma/2  $.
The total possibilities of the unique blocks is $2^{r_1 k'}$.
The number of combinations of  positions of unique blocks in non-zero blocks is $ {r \choose r_1} $.
Let the number of non-removed positions in non-unique nonzero blocks of $w$ and $u$, without duplicates, be $ m_3 $.
For bits at these positions there are $2^{m_3}$ possibilities, because by \cref{lem:conditionuniform}, we do not have to count other codewords which are in the same coset.
Recall the number of different positions of zero blocks in $w$ and $u$ is ${2t+1 \choose r}$.
So the total number is ${2t+1 \choose r} {r \choose r_1} 2^{r_1 k'}  2^{m_3} $.

Notice that $ (2t+1)n' - 2m_1 - 2m_2 - 2m_3 \ge  r_1 n'$, since we   only remove symbols in zero blocks, symbols in non-unique blocks and those $m_3$ bits that are  in non-unique blocks.
So  $   tn_0 - m_1 - m_2 - d' - m_3\ge  (r_1-1)n'/2- d'$.
Notice that 
\begin{align}
    & 2^{-(r_1-1)n'/2+ d'} {2t+1 \choose r} {r \choose r_1} 2^{r_1 k'} \\
<   & 2^{-(r_1-1)n'/2+ d'} \left( \frac{e(2t+1)}{r} \right)^r \left( \frac{e r}{r_1} \right)^{r_1} 2^{r_1 k'} \\
<   & 1
\end{align}
if we take $k' = (\frac{1}{2} - \gamma/2)n', k' = \log q = \frac{6}{\gamma}\log n $, $ r_1 \gamma/2  > 2 $.
Note that $ r_1 \gamma/2  > 2 $ as long as $ s \ge 5/\gamma $.


Now we derandomize the construction.
Next we replace uniform randomness by an $\eps_0$-bias distribution with $\eps_1 = 2^{-c_1 \log n}$, with constant $c_1$ large enough.
Notice that by Theorem \ref{}, the seed length is $O(\log n)$.
Consider $M'$.
We focus on all positions, in non-zero blocks, that appear in pairs of $M'$.
Denote the bits at these positions as a sequence $u$.
Notice that each bit in $u$ is a linear function of the $\eps_0$-bias distribution, and all these linear functions are linear independent.
Also $|u| \le rn' = O(\log n)$, since every pair of $M'$ has one entry which is from a non-zero block and $M'$ is monotone.
When $c_1$ is large enough,   by the XOR lemma, the bits of $u$, is $\le \eps \eps_0 2^{ |u|/2}$ close to uniform.
So the probability is $\le 2^{-M'} + \eps \eps_0 2^{ |u|/2}$ which is at most $2^{-M'+1}$ when $c_1$ is large enough.
The remaining analysis can still go through.



\end{proof}



\begin{lemma}
\label{lem:conditionuniform}
For every integer $t\le k$,
let $\vec{a}_1, \vec{a}_2, \ldots, \ldots, \vec{a}_k $ be uniform  random vectors over $\{0, 1\}^{n}$.
Let $A \in \{0, 1\}^{n\times k}$ be the matrix such that its $i$-th column is $\vec{a}_i$.
For every set of $t$ linearly independent vectors $\vec{x}_1, \ldots, \vec{x}_t$ over $\{0, 1\}^k$,
for every set $S\subseteq  [n]$ of size $k-t$,
conditioned on that the $S$-kernel of $A$ is the space $span(\vec{x}_1, \ldots, \vec{x}_t)$,
for every  $ \vec{y} \in  \{0, 1\}^k \setminus span(\vec{x}_1, \ldots, \vec{x}_t)$, every $\vec{z} \in span(\vec{x}_1, \ldots, \vec{x}_t)$,
it holds that $A (\vec{y}+\vec{z})|_S$ is uniform.
\end{lemma}
Here $span(\vec{x}_1, \ldots, \vec{x}_t)$ is linear space spanned by $\vec{x}_1, \ldots, \vec{x}_t$.
\begin{proof}
Since $\vec{x}_1, \ldots, \vec{x}_t$ are linearly independent, if we solve the linear system $A \vec{x}_i |_S = 0, \forall i\in [t]$, regarding $\vec{a}_1, \ldots, \vec{a}_k$ as variables, then the number of free variables is $ k-t $ while non-free variables can all be written as linear combinations of free variables.

So conditioned on that the $S$-kernel of $A$ is the space $span(\vec{x}_1, \ldots, \vec{x}_t)$, the distribution $A$ can be viewed as such that all free variables are independent and uniform random, while non-free variables restricted on $S$ are linearly dependent on free variables restricted on $S$. 
This linear dependence is exactly the solution of the linear system.

For every  $ \vec{y} \in  \{0, 1\}^k \setminus span(\vec{x}_1, \ldots, \vec{x}_t)$, every $\vec{z} \in span(\vec{x}_1, \ldots,\vec{x}_t)$, we know that $A (\vec{y}+\vec{z})|_S = A \vec{y}|_S$.
Further, since $\vec{y}$ is not in $span(\vec{x}_1, \ldots, \vec{x}_t)$, $A \vec{y}|_S$ is a non-zero linear combination of free variables.
So it is uniform.

\end{proof}

\subsection{Efficient decoding}

Let $\corrupted$ be a corrupted codeword with   at most $ t = O(  N) $ insdel errors.
%Let $f(i, j)$ denote the length of a common sequence, between the first $i$ blocks and the first $j$ symbols in $y$, defined as the following.

We  first define the following functions $g$.
For every $v\in \alphabetin^*$ and $i, i'\in [n]$, we let
\[g([i', i], v) = \begin{cases}
1, \text{ if } \exists u \in \bigcirc_{j=i'}^{i}\Cin^j  \text{ s.t. } \ell := \lcs(u,v) \ge |u| + |v| - d'/2 \text{ and } u  \text{ has exactly } s \text{ non-zero blocks}, \\
0, \text{ otherwise.}
\end{cases}
\]
We call such a match $(v, [i, i'])$ with $g(v, [i, i']) > 0$, as a segment match.
Also we call $u$ as a candidate for match.
Denote the sequence of non-overlapping segment matches as a segment matching.
Let $f[i, j]$ be the size of the longest segment matchings between the first $i$ blocks and the first $j$ symbols of $\corrupted$.

We use the following dynamic programming to compute $f[i, j]$.
Let $f[i,j] = 0$ if $i = 0 $ or $j = 0$. 
For $1\le i \le n$ and $1\le j \le N$, we can compute $f[i,j]$ using the following transition rule:
\[f[i,j] = 
\underset{0\le j'<j, 0\le i' < i}{\max} \; f[i', j'] + g([i', i], \corrupted_{[j'+1: j]}).
\]
One can compute the corresponding matching along with the computing of $f[i, j]$.
Denote this matching as $M$.

Next, the decoder recovers all the blocks according to $M$.
Then assign zeros to all the other blocks.


Recall that $\corrupted$ is a corrupted version of $z$.
Denote $z_0$ as the outer codeword of the original message $x$.
\begin{lemma}
\label{lem:ellLB}
The longest segment matching between $z$ and $\corrupted$ has size $\ell$ at least $ \lfloor w(z_0)/s\rfloor - \frac{\rho nn'}{d'/2 }$.

\end{lemma}

\begin{proof}

We cut $u$ into a sequence of consecutive blocks, such that each segment contains exactly $s$ non-zero blocks.
The number of such segment is at least $ \lfloor\frac{w(z_0)}{s}\rfloor  $.
Now consider these segments which do not have more than $d'/2$ insdels, the number of which is at least $l =  \lfloor\frac{w(z_0)}{s}\rfloor - 2\rho nn'/ d' $.


\end{proof}

\begin{lemma}
\label{lem:longSegmentMatching}
$f[n, |\corrupted|] \ge \ell$
\end{lemma}
\begin{proof}
We only need to show the claim that $f[i, j]$ is   the size of the longest common segment matching between the first $i$ blocks and the first $j$ symbols of $\corrupted$.

If $i=0$ or $j=0$, then it's obvious that this is true.

Assume the this is true for every $f[i', j'], i' \le i, j'\le j$.
Consider $f[i+1, j]$.
Consider the longest common segment matching is actually $M$. 
Without loss of generality assume its size is not $0$.
Assume the first $|M|-1$ segment matches are between the first $i^*$ blocks and the first $j^*$ symbols of $\corrupted$.
Then we know that $|M| \le f[i^*, j^*] + 1$.
Notice that this is at most $f[i, j]$.

In the same way one can show that $f[i, j+1]$ is also the maximum.

So the claim is true.


\end{proof}

Now consider every segment  match $( [i, j], v  )$ in $M$.
Call the interval $v$ good if the number of inserted symbols and the number of deleted symbols (between the first undeleted symbol and the last undeleted symbol) is   $<d'/2$.


\begin{lemma}
\label{lem:goodSubstr}
For every segment match $( [i, j], v )$  in $M$, if $  v $ is good, then $u$ has  at most $ O(\gamma )s$ blocks different  from the corresponding blocks of $z$.
\end{lemma}

\begin{proof}
Let $u$ be the candidate string for  $( [i, j], v )$.
Consider the sequence of consecutive blocks $w$ starting from the one which includes the first undelete symbol in $\corrupted$, to the one which includes the last undeleted symbol in $\corrupted$.

Notice that the number of blocks in $w$ is at most the number of blocks in $u$ plus 2. 
Since otherwise, the insdel distance between $u$ and $v$ cannot be at most $d'/2$.

Also as $u$ has $s$ non-zero blocks, the total number of non-zero blocks in $v$ is   at most $s+O(1)$.
Since otherwise, the insdel distance between $u,v$ has to be at least $d'$.

When $[i, j]$ is good, by \cref{prop:propertymain-s}, as  $(  [i, j], v)$ is a segment match, it has to be that  the number of unique blocks in $u$, comparing to $w$, is at most $O(\gamma s)$.

\end{proof} 


\begin{lemma}
The decoder can successfully decode $x$ when there are $\le \rho $ fraction of errors.
\end{lemma}

\begin{proof}

By \cref{lem:longSegmentMatching}, the segment matching $M$ has size at least $\ell$.
Notice that there are at most $b = \frac{\rho nn'}{d'/2}$ substrings in the matching being not good.
So the remaining $\ell -b  $ substrings are all good.
Then by \cref{lem:goodSubstr}, the number of correctly recovered blocks is at least $  s(1-O(\gamma )(\ell - b)  $.
By the lower bound of $\ell$ from \cref{lem:ellLB}, we know this is  at least $ w(z_0) -1 -   2s\frac{\rho nn'}{d'/2}$

\end{proof}

==> construction_hrate_old.tex <==
\section{Constructions with High Rate}
In this section, we first give our linear codes with a rate arbitrarily close to $1/3$, which can still correct a constant fraction of insdel errors.


\paragraph{The construction.} Following our general construction, here we take $\Cout$ to be an $[n,k,d]_n$ Reed-Solomon code with alphabet size $|\alphabetout| = n$, $k = (1- \delta) n$ and $d = \delta  n$ for some constant $\delta>0$ to be chosen later. We construct $n$ different inner codes $\Cin^1, \dots, \Cin^n$ with   alphabet size $2$, message length $k'= \log n = (\frac{1}{3}-\beta)n'$ such that they satisfy the following property.



\begin{property}\label{prop:propertymainbasic}
  
  %\item $\forall i \in [n]$, $\Cin^i:\alphabetout \rightarrow \alphabetin^{n'} $ is a linear code with rate $\gamma_i = $.
 \iffalse 
  \begin{enumerate}
  \item $\forall i\in[n]$, $\forall u, v \in \Cin^i$, if $u\neq v$, then $\ed(u,v) \ge d'$.
  
  \item $\forall i, j \in [n], i\neq j$,   $\forall u\in \Cin^i, v \in \Cin^j$, if $u$ and $v$ are not both $0^{n'}$, then $\ed(u,v) \ge d'$. 
  
  \item $\forall i \in [n], j \in [n-1]$, $\forall w\in \Cin^i, u\in \Cin^j, v\in \Cin^{j+1}$, if $w\neq u$ and $w \neq v$, then for any substring $ w' $ of $u\circ v$, we have $\ed(w, w')\ge d'$.
  
 % Let $u,v,w \in \cup_{i = 1}^n\Cin^i$. If $w\neq u$ and $w\neq v$, then for any substring $w'$ of $u\circ v$, we have $\ed(w, w')\ge d'$.
\end{enumerate}
\fi

 $\forall i \in [n], j \in [n-1]$, $\forall w\in \Cin^i, u\in \Cin^j, v\in \Cin^{j+1}$,
\begin{enumerate}

    \item except that $w = u $ or $w = v $, it always holds that for any substring $ w' $ of $u\circ v$, we have $\ed(w, w')\ge d'$;
    
    \item if  $u = 0^{n'}, v \neq  0^{n'}$ (resp. $v = 0^{n'}, u \neq 0^{n'}$) and $w = 0^{n'}$, then for any substring $w'$  of $u\circ v$, which has  $\le 2n'/3  $ bits overlapping with $u$ (resp. $v$), we have $\ed(w, w') \ge d'$.  
        
\end{enumerate}
   
 

\end{property}
\xnote{The above statement in the current form is false. What if $i=j$ and $w =u \neq 0^{n'}$?}
We show the following about the inner codes. 
\iffalse
\begin{lemma}
%$\forall \ n$ and $|\alphabetout| = \Theta(n)$ and $ |\alphabetin| = O(1)$, there exists $ n' = \Theta(\log(n))$ and $ d' = \Theta(n')$, such that 
There exists $\Cin^1, \dots, \Cin^n$ such that:
\begin{enumerate}
    \item $\forall i \in [n]$, $\Cin^i:\alphabetout \rightarrow \alphabetin^{n'} $ is a linear code with rate $\gamma_i = $. 
    \item $\forall i \in [n]$, $\Cin^i $ is an insdel code with edit distance $d'$. i.e. $\forall i \in [n]$, any two distinct codewords $u,v \in \Cin^i,$ must have $\ed(u,v) \ge d'$. 
   \item Let $u,v,w \in \cup_{i = 1}^n\Cin^i$. If $w\neq u$ and $w\neq v$, then for any substring $w'$ of $u\circ v$, we have $\ed(w, w')\ge d'$.
%    \item $\forall u, v, w \in \cup_{i = 1}^n\Cin^i$, with

\end{enumerate}
\end{lemma}
\fi

\begin{lemma}
For every $d' \in \mathbb{N}$, , there exists an efficient construction of $n$ inner codes $\Cin^1, \dots, \Cin^n$ satisfying \cref{prop:propertymainbasic} with parameter $d'$, where each $\Cin^i$ has alphabet size $2$, rate $\gamma_i =  \frac{1}{3}-\eta $, for every $\eta \geq  \frac{ d'}{ n'} \log \frac{ e(n'+d')}{d'}$.
\end{lemma}
\xnote{If we write $\eta \geq ...$ then we only get the rate $\gamma_i \leq ...$, but we actually need the rate to be as large as possible.}

\xnote{In this basic case we cannot hope to get rate close to $1/2$ for the inner codes. We can only get close to $1/3$.}

\begin{proof}
We first show that a random construction suffices and then show how to derandomize it.

For every $i$, the random construction  independently chooses a random basis of dimension $(\frac{1}{3}-\gamma')n'$ for $\Cin^i$. 
Then it checks if these codes meet \cref{prop:propertymainbasic}.
%Notice that the whole procedure is in time $\poly(n)$.

Consider the first item in \cref{prop:propertymainbasic}.
If  $ \ed(w, w') \le d' $, then $\lcs(w, w') \geq  (n' + |w'|-d')/2$.
Since every base vector is independently randomly chosen, a fixed matching of size $ m =  (n' + |w'|-d')/2$ with all matches correct, happens with probability at most $ 2^{-m} $.
There are at most ${n'\choose m}\cdot {|w'|\choose m}  $ such matchings.
There are $ 2^{3k'}$ different triple $(w, u, v)$.
And there are at most $(2n'-d')\times 2d' \le 4n'd'$ different $w'$, i.e. only consider $w'$ with length in $[n'-d', n'+d']$ is sufficient.
Hence  \cref{prop:propertymainbasic} item 1 does not happen with probability at most 
\begin{align}
  {n'\choose m}\cdot {|w'|\choose m}  2^{3 k' } 4n'd'  2^{-m}  
  &= {n'\choose n'-m} {|w'|\choose |w'|-m} 2^{3 k'} 4n'd' 2^{-m} \\
 &\le \left( \frac{en'}{d' } \right)^{d' }  \left( \frac{e(n'+d')}{d'} \right)^{d'}  2^{3(1/3-\eta)n'} 4n'd' 2^{-(n'-d')}.
\end{align}
When $\eta \geq \frac{ d'}{ n'} \log \frac{ e(n'+d')}{d'}$, this is $ < 0.1$.

Consider the second item in \cref{prop:propertymainbasic}.
Denote the part of $w'$ which does not overlap with $u$ as $w''$.
If $ \ed(w, w') \le d' $, then    $ \lcs(w, w'') \ge (n' + |w'|-d')/2 - 2n'/3 $.
Notice that for $v$ (resp. $u$) its corresponding base vectors are independently chosen.
So again a fixed matching of size $ m =  (n' + |w'|-d')/2 - 2n'/3 $ with all matches correct, happens with probability at most $ 2^{-m} $.
There are also at most ${n'\choose m}\cdot {|w'|\choose m}  $ such matchings.
But there are $2^{k'}$ different triple $(w, u, v)$, since $w$ and $u$ (resp. $v$) are zero codewords.
And there are at most $4n'/3 \times 2d' \le 4n'd'$ different $w'$, i.e. only consider $w'$ with length in $[n'-d', n'+d']$ is sufficient.
Hence  \cref{prop:propertymainbasic} item 2 does not happen with probability at most 
\begin{align}
  {n'\choose m}\cdot {|w'|\choose m}  2^{ k' } 4n'd'  2^{-m}  
  &= {n'\choose n'-m} {|w'|\choose |w'|-m} 2^{ k'} 4n'd' 2^{-m} \\
 &\le \left( \frac{en'}{d' } \right)^{d' }  \left( \frac{e(n'+d')}{d'} \right)^{d'}  2^{(1/3-\eta)n'} 4n'd' 2^{-(n'/3-d')}.
\end{align}
When $\eta \geq \frac{ d'}{ n'} \log \frac{ e(n'+d')}{d'}$, this is $ < 0.1 $.

By a union bound, the outcome of the random generating process can meet \cref{prop:propertymainbasic} with a constant probability. 
And the checking procedure can find out the desired outcome.
\xnote{no need to find the ``desired outcome" in the random construction.}

Next we replace uniform randomness by $\eps$-biased distribution $r $ over $\{0, 1\}^{k'n'n}$ from  , 
\knote{Need a prelim theorem for pseudorandomness.} with $\eps = 2^{-3m}$.
Notice that the seed length is $O(\log n)$.
So finally we can try all seeds and find out a desired outcome.
In the above proof,  we consider a fixed matching $M$ between $w$ and $ w'$.
Now we focus on the  bits in pairs of $M$.
Denote them as a string $s$.
Notice $|s| \leq 2m$.
Each   bit of $s$ is linear in bits of $r$.
So an XOR of any their subset is $\eps$-biased from uniform.
By the XOR Lemma, $s$ is $\eps \cdot \sqrt{2^{2m}} = 2^{-2m}$-close to uniform.
So $M$ has all its matches being correct with probability $\leq 2^{-m}+ 2^{-2m}$ instead of $2^{-m}$. 
The above analysis can still go through when this is the case.
\end{proof}



\subsection{Decoding via Dynamic Programming}
\xnote{I used $z$ to denote the uncorrupted codeword and $y$ to denote the received word. Perhaps better to be consistent here.}
We now show how to decode $\C$ from insdel error via dynamic programming. For convenience, we let $N = n\cdot n'$. Let $x\in \alphabetout^k$ be the original message, $z \in \C(x)$ be the uncorrupted codeword. We can view $z$ as $z^1\circ z^2 \circ \cdots \circ z^n$ where each $z^i$ is a codeword of $\Cin^i$. 

\xnote{I believe for the DP, we can use the same objective function as in Section 4, i.e., minimizing the total insdel distance or maximizing the total LCS, instead of setting a threshold of $d'/2$ and then maximizing the number of matches above this threshold. This will unify our decoding algorithms. Although, we probably don't have enough time to make these changes.}
Let $\corrupted$ denote the corrupted codeword. For any substring $\corrupted_{[j:k]}$ of $\corrupted$, we say it can be matched to $i$-th position if $\ed(\corrupted_{[j:k]}, u)\le d'/2$ for some $u\in \Cin^i$. We can define the following functions $g_i$ for each $i\in [n]$ to denote whether a string $u$ can be matched to the $i$-th position, i.e. for any $v\in \alphabetin^*$ and $i\in [n]$, we let

\[g_i(v) = \begin{cases}
1, \text{ if } \exists \ u \in \Cin^i, \text{ s.t. }\ed(u,v) \le d'/2, \\
0, \text{ otherwise.}
\end{cases}
\]


For any $i\in [n]$ and $j\in [N]$, we say there is an alignment of size $k$ between $\corrupted_{[1:j]}$ and the first $i$ positions if we can find $k$ non-overlapping substrings $\corrupted_{[\alpha_1: \beta_1]}, \dots,  \corrupted_{[\alpha_k: \beta_k]}$, $1\leq \alpha_1\leq \beta_1 \le \cdots \le \alpha_k \le \beta_k \le j$, and $k$ indices $1\le t_1< \dots< t_k\le i$ such that   $ g_{t_l}(\corrupted_{[\alpha_l: \beta_l]}) = 1$ for $l\in [k]$.

\xnote{Before the details of DP, we need to first explicitly say what is the objective function we are trying to optimize.}

The dynamic programming computes the maximum size of alignments between  $\corrupted$ and the first $n$ positions. It proceeds by computing a matrix $f$ such that $f[i,j]$ is the size of the largest alignment between $\corrupted_{[1:j]}$ and the first $i$ positions. We let $f[i,j] = 0$ if $i = 0 $ or $j = 0$. For $1\le i \le n$ and $1\le j \le N$, we can compute $f[i,j]$ using the following updating rule:

\[f[i,j] = 
\max \begin{cases}
\underset{0\le j'<j}{\max} \; f[i-1, j'] + g_i(\corrupted_{[j'+1: j]}), \\
f[i, j-1].
\end{cases}
\]

Each value $f[i,j]$ corresponds an canonical alignment, denoted by $M[i,j]$. $M[i,j]$ has size $f[i,j]$ and can be represented as $M[i,j] = \left( (t_1, \corrupted_{[\alpha_1: \beta_1]}), \dots, (t_k, \corrupted_{[\alpha_k: \beta_k]})\right)$ where $k = f[i,j]$. Each tuple $(t_l, \corrupted_{[\alpha_l: \beta_l]})$ represents a match  from the substring $\corrupted_{[\alpha_l: \beta_l]}$ to the $t_l$-th position in the correct codeword. Thus, for any $l\in [k]$, we have $g_{t_l}(\corrupted_{[\alpha_l: \beta_l]}) = 1$. 

Specifically, $M[i,j]$ is constructed as following. For $i=0$ or $j=0$, $M[i,j]$ is empty. For $i,j$ both nonzero, if $f[i,j] = f[i, j-1]$, then $M[i,j] = M[i,j-1]$. Otherwise, $f[i,j] = f[i-1, j'] + g_i(\corrupted_{[j'+1, j]})$ for some $0 \le j' < j$. If there are multiple such $j'$, we choose an arbitrary one. Then, if $g_i(\corrupted_{[j'+1: j]}) = 1$, we append $(i, \corrupted_{[j'+1: j]})$ to $M[i,j']$ to get $M[i,j]$. If  $g_i(\corrupted_{[j'+1: j]}) = 0$, we let $M[i,j] = M[i,j']$.

\subsection{Analysis}


\begin{claim}
\label{claim:alignment_size1}
Any alignment between $\corrupted_{[1:j]}$ and the first $i$ positions has size at most $f[i,j]$.
\end{claim}

\begin{proof}
We prove this by induction on $i$ and $j$. The base case is $i=0$ or $j=0$. We have $f[i,j] = 0$ by definition. The claim holds trivially. For fixed $0 < i_0 < n$ and $0 < j_0 < N$, we assume the claim holds for any $i,j$ such that $0\le i \le i_0$ and $0 \le j \le j_0$. We show that the claim also holds for $f[i_0 + 1, j_0]$ and $f[i_0, j_0 + 1]$. 

For $f[i_0+1, j_0]$, let $M'$ be an optimal alignment between $\corrupted_{[1:j_0]}$ and the first $i_0 + 1$ positions. There are two cases. First, there is a match  $(i_0+1, \corrupted_{[j' + 1:j_0]})$ in $M'$ for some $j'$. Then $M'\setminus \{(i_0 + 1, \corrupted_{[j': j_0]})\}$ is a matching between $\corrupted_{[1:j']}$ and the first $i_0$ positions.  Since  $\forall j', f[i_0, j']$ is the size of the largest alignment between $\corrupted_{[1:j']}$ and the first $i_0$ positions by the inductive hypothesis, we know $  f[i_0, j'] + 1 = |M'| $.
Thus $f[i_0+1, j_0] \ge f[i_0, j'] + 1 =  M'$. 
The second case is when there is no matching between any substring to $(i_0 + 1)$-th position in $M'$. Then $M'$ is an alignment between $\corrupted_{[1: j_0]}$ to the first $i_0$ positions. By the inductive hypothesis, we have $|M'| =  f[i_0, j_0]$. By the updating rule of $f$, we have $f[i_0 + 1, j_0]\ge f[i_0, j_0]$.
So $f[i_0 + 1, j_0]\ge |M'|$.

The proof is similar for $f[i_0, j_0 + 1]$. 

\end{proof}




%Specifically, $\corrupted_{[\alpha_1: \beta_1]}, \dots,  \corrupted_{[\alpha_k: \beta_k]}$ are $k$ non-overlapping substrings of $\corrupted$ such that $\corrupted_{[\alpha_l: \beta_l]}$ is to the left of  $\corrupted_{[\alpha_{l+1}: \beta_{l+1}]}$ (i.e. $\beta_l < \alpha_{l+1}$) for any $ l \in [k-1]$. $t_1,\dots t_k$ are indices such that $1\leq t_1 < \cdots < t_k \leq i$. Each tuple $(\corrupted_{[\alpha_l: \beta_l]}, t_l)$ represents a match from the substring $\corrupted_{[\alpha_l: \beta_l]}$ to the $t_l$-th position in the correct codeword. For any $l\in [k]$, we have $g_{t_l}(\corrupted_{[\alpha_l: \beta_l]}) = 1$. 

In the following discussion, we assume $\ed(z, \corrupted) = T$. \xnote{the same string $y$?}
We first show the following claim. 

\begin{claim}
\label{claim:alignment_size2}
$f[n, N] \ge n-2\frac{T}{d'}$.
\end{claim}

\begin{proof}
We show that there is an alignment between $\corrupted$ and the $n$ positions with size $n-2\frac{T}{d'}$. Then the claim is a direct result of \cref{claim:alignment_size1}. 

Since $\ed(z, \corrupted) = T$, there is a sequence of $T$ edit operations that transforms $z$ to $\corrupted$. \xnote{again, the same $y$. Should change $y$ to $z$} Denote $z = z^1\circ \cdots \circ z^n$, where $z_i \in \Cin^i, i\in [n]$. The $T$ edit operations can be partitioned into $n$ groups such that the $i$-th group of the edit operations is performed on $z^i$.  Notice that there are at most $2\frac{T}{d'}$ groups with more than $d'/2$ edit operations. Thus, for the remaining positions, $\ed(z^i, \corrupted^i)\le d'/2$. For these positions, $\corrupted^i$ can be matched to $i$-th position. This gives an alignment of size at least $n-2\frac{T}{d'}$.
\end{proof}

For any match $(\corrupted_{[\alpha:\beta]}, t)$, we say it is a correct match if $\ed(\corrupted_{[\alpha:\beta]}, z^t)\le d'/2$. Otherwise, we say it is a wrong match. 
The set of matches found by the dynamic programming may contain wrong matches. The following lemma ensures that we can find a good amount of correct matches. 

\begin{lemma}
The number of correct matches in $M[n, N]$ is at least $n-8\frac{T}{d'}$.
\end{lemma}


\begin{proof}

We assume $M[n,N] $ has size $m$ i.e.
\[
M[n,N] = \left( (t_1, \corrupted_{[\alpha_1: \beta_1]}),(t_2, \corrupted_{[\alpha_2: \beta_2]}), \dots, (t_m, \corrupted_{[\alpha_m: \beta_m]})\right).
\]
 In other words, the dynamic programming finds $m$ non-crossing matches such that the substring $\corrupted_{[\alpha_i: \beta_i]}$ is matched to the $t_i$-th position. 

Our goal is to show that among these $m$ matches, at least $n-10\frac{T}{d'}$ are correct match. In the following analysis, we fix a set of $T$ edit operations that transform $y$ to $\corrupted$. 

Before the proof, we first give some definitions. 

We say a symbol in $\corrupted$ is an original symbol if it is not an inserted symbol. For any $1\le \alpha < \beta \le N$ and the substring $\corrupted_{[\alpha:\beta]}$, let $\alpha'$ be the index of the first original symbol in $\corrupted_{[\alpha:\beta]}$ in the original codeword $z$ and $\beta'$ be the index of the last original symbol in $\corrupted_{[\alpha:\beta]}$ in the original codeword $z$. We say $z_{[\alpha':\beta']}$ is the substring in $z$ that is corresponding to $\corrupted_{[\alpha:\beta]}$. It is possible that $\alpha'=\beta'$ is there is only 1 original symbol in $\corrupted_{[\alpha:\beta]}$. If there is no original symbol in $\corrupted_{[\alpha:\beta]}$, then the corresponding substring in $z$ is empty. 

Under this definition, for each substring $\corrupted_{[\alpha_l: \beta_l]} $, there is a substring $z_{[\alpha'_l: \beta'_l]}$ in $z$ that corresponds to it. We denote $T_l= \ed(\corrupted_{[\alpha_l: \beta_l]},z_{[\alpha'_l: \beta'_l]} )$. 


For each match $(t_l, \corrupted_{[\alpha_l: \beta_l]})$, we let $u^{t_l}\in \Cin^{t_l}$ be the codeword such that $\ed(u^{t_l}, \corrupted_{[\alpha_l: \beta_l]}) \le d'/ 2$. The match is either a correct match or a wrong match ($u^{t_l}=z^{t_l}$ or $u^{t_l}\neq z^{t_l}$). 

For wrong matches, we consider $T_l$.
There are two cases.
First, $T_l > d'/2$. This is the case when a lot of edit operations happen in the substring. It could be matched to a wrong position. Second, $T_l \le d'/2$. By \cref{prop:propertymainbasic}, the only possible case is that $u^{t_l} = 0^n$. \xnote{The only possible case of a wrong match? Otherwise doesn't make sense.}This is because $0^n$ is a codeword of all inner codes. It is possible that we match a substring of $\corrupted$ close to $0^n$ to a wrong position. Thus, we can divide our matches in $M[n,N]$ into the following 3 cases. 

\iffalse
\begin{itemize}
    \item Type 1: Correct matches with $T_l > d'/2$.

    \item Type 2: Correct matches with $T_l \le d'/2$.
    
    \item Type 3: Wrong matches with $T_l > d'/2$. 
    
    \item Type 4: Wrong matches with $T_l \le d'/2$.
    
\end{itemize}
\fi
\begin{itemize}
    \item Type 1: Correct matches.
    
    \item Type 2: Wrong matches with $T_l > d'/2$. 
    
    \item Type 3: Wrong matches with $T_l \le d'/2$.
    
\end{itemize}

Let $m_i$ be the number of type $i$ matches for $i=1,2,3$. We have $m=m_1+m_2+m_3$.

Since there are a total of $T$ edit operations. Each type2 match corresponds to more than $d'/2$ edit operations. We have the following claim. 

\begin{claim}
\label{clm:wrong_match}
 $m_2 \le 2\frac{T}{d'}$.
\end{claim}

We now prove an upper bound of $m_3$.

\begin{claim}
\label{clm:zero_match}
% $m_4 \le 4\frac{T}{d'}$. 
$m_3\le 4\frac{T}{d'}$. 
\end{claim}






We have $m=m_1+m_2+m_3  \ge n-2\frac{T}{d'}$ by \cref{claim:alignment_size2}. The lemma follows directly from \cref{clm:wrong_match} and \cref{clm:zero_match}.


\end{proof}


Before we show the proof of \cref{prop:propertymainbasic}, we introduce some more notations. 
The corrupted codeword $\corrupted$ can be partitioned into $t$ segments, i.e. $\corrupted = \corrupted^1 \circ \cdots \corrupted^2$, such that $\corrupted^i$ starts from the first non-deleted symbol in $z^i$ and includes all the symbols before (not include) the first symbol of $z^{i+1}$.
If all symbols in $z^i$ are deleted then $\corrupted^i$ is an empty string.
If $i$ is the largest such that not all symbols in $z^i$ is deleted, then it includes all the symbols to the right end of the string.
If $i$ is the smallest such that not all symbols in $z^i$ is deleted, then $\corrupted^i$ further includes all the symbols to the left of the first symbol in $z^i$.
By saying a segment $\corrupted^i$ has $k$ insdel operations, we mean it takes $k$ insdels to transform to it from $z^i$.


\subsection{Proof of \cref{clm:zero_match}}
We show that for each such match, one can map it to either a unmatched block in $z$  or a block in $z$ which is corrupted by at least $d'/10$ insdels.\xnote{Without repetition?}
Moreover, in this map, each unmatched block in $z$ has at most 1 preimage and each block in $z$ with $\ge d'/10$ insdels has at most $ 2 $ preimages.
%For each output of $A$, there are at most $3$ inputs having the same output.

But before prove the claim we need to show the followings.

\begin{claim}
Each $I$ in a match in $M$ overlaps with at most $2$ (consecutive) segments.
\end{claim}
\begin{proof}
Suppose not.
Notice that $|I|$ has to be at most $n'+d'/2$, since otherwise it cannot have distance $\le d'/2$ with any inner codewords.
First suppose $I$ has overlaps with $\ge 4$ consecutive segments and we only consider the first $4$ of them.
Then the two segments in the middle must have   $>n' - d'/2$ deletions, otherwise $I$ cannot overlap with $4$ segments.
Then one of them has to have  $  > (n' - d'/2)/2 \geq d'/10$ deletions, when $d' \le \frac{10}{7}n'$. 
So $|I|$ only has overlaps with $\le 3$ consecutive segments.
However if there are three consecutive blocks, then either the left  one  or the right one has overlaps of size  $< 3d'/10$ with $I$.
This is because the segment in the middle should have length   $> n'-d'/10$ and $|I| \le n'+d'/2$.
In average one of the remaining two should have an overlap of size $< 3d'/10$ with $I$.
Without loss of generality, assume it is the left one.
Notice that we are considering a wrong match with $T_l \le d'/2$.
Hence it must holds that $I$ is within distance $\le d'/2$ to $0^{n'}$, otherwise by \cref{prop:propertymainbasic} the distance is $\ge d'$.
Also by \cref{prop:propertymainbasic}, the overlap between $I$ and the remaining two segments (the middle one and the right one), has distance   $>d' - 2\cdot d'/10 = 4d'/5$ from $z^t$.
So the overall distance is   $> 4d'/5 - 3d'/10 \ge d'/2$.
This is a contradiction.
\end{proof}


\paragraph{The map $A$}
The map is established using the following algorithm $A$.
The input is a match $(t_l, \corrupted_{[\alpha_l:\beta_l]})$ from the matching $M$.
$A$ has a finite number of rounds and  maintains an index $t$ corresponding to a block in $z$ and a interval $I$ which corresponds to a substring in $\corrupted$.
At the beginning of the first round, $t$ is set to be $t_l$, and $I$ is set to be $ \corrupted_{[\alpha_l:\beta_l]}$.
Consider the $i$-th round.
We know that $I$ has overlaps with at least $1$ segment. If any of them is under  $\ge d'/10$ corruptions, then $A$ outputs this block. 
Otherwise we do the following.






\begin{claim}
Consider the  corresponding blocks in $z$ of these two segments as $b_1, b_2$.
At least one of $b_1, b_2$ is the $0$ codeword.
\end{claim}
\begin{proof}
Notice that the total number of corruptions in these two segments is $< 2\cdot d'/10 \le d'/2$.
Recall we showed that $I$ is within distance $\le d'/2$ to $0^{n'}$.
Hence by \cref{prop:propertymainbasic}, at least one of $b_1, b_2$ is $0$.
\end{proof}


\paragraph{The map $A$ (continuous)}
The algorithm picks one of $b_1, b_2$ by the following criteria.
If $I$ has overlaps with one segment for $> 2n'/3-d'/5$ bits then pick that one.
Otherwise pick the right one.
%It first checks the number of bits that $I$ inherited from block $b_1$ and $b_2$.
%Pick the one which it inherits more bits.
%If there is a tie, then pick the rightmost block.
Then it renews $t$ to denote this block.
If there is no match in the matching which is matched to  $z^t$, then $A$ outputs $t$.
Otherwise, assume there is such a match, then $A$ sets $I$ to be the interval of $\corrupted$ in this match.
This is the end of the current round.


Now we show that starting from two distinct type-3 matches $w, w'$, the two runs $A(w)$ and $A(w')$ do not have the same value of $t$ in any of their rounds $i, i'$. 

Suppose not.
Denote the block index variables used  in the two runs as $t, t'$, and the interval variables used in the two runs as $I, I'$. 
Assume the two runs have $t= t' = t_0$ at the beginning of their $i, i'$-th rounds respectively, with $i$ being the smallest such $i$. 
It is impossible that $i = 1 $ or $i' = 1$, since we start from two different matches.
Without loss of generality assume $i = 1$. 
Then $i' >1$, since otherwise $w = w'$.
This means $z^t$ has to be $0$, because in the $i'-1$-th round  $t'$ is picked by $A$ (Recall $A$ only picks zero blocks).
But when $z^t$ is $0$,  $w$ can not be a type-3 match.
So the only case we need to analyze is $i, i' > 1$.

Consider $I$ and $I'$ at the beginning of their $i-1, i'-1$ rounds respectively.
Then $I$ and $I'$ have to be different, since otherwise $i$ is not the smallest one that $t = t'$.
Notice that $I$ and $I'$ have no overlaps due to that they are   from  distinct matches of $M$.
By the definition of $A$, in order to have $t = t'$ at the beginning of their round $i, i'$, it must holds that $I$ and $I'$ have overlaps with a same segment $t_0 = t = t'$.
Without loss of generality, assume $I$ is to the left of $I'$.
By the definition of $A$, as $A(w)$ picks $t = b_2 $, there are 2 possibilities.

First $I$ overlaps with $\corrupted^t$ for   $> 2n'/3 - d'/5 $ bits.
Then $A(w')$ cannot choose $t_0$ since it does not has $> 2n'/3 - d'/5 $ bits overlapping with $\corrupted^t$.
Second $I$   overlaps with $\corrupted^t$ for   $\le 2n'/3 - d'/5 $ bits.
Then we show that both 

First its $b_1$ is not a zero codeword. 
In this case, $I$ has to have overlaps with $\corrupted^t$ for  $> 2n'/3 - d'/5 $ bits.
This is because if the overlapping size is $\le 2n'/3 -d'/5$, then since there are  $\le d'/5$ insdels inside $z^{t-1}\circ z^{t}$, one can use $d'/5$ insdels to transform $I$ to be a  interval  $\tilde{I}$  of $z^{t-1}\circ z^{t}$ such that $|\tilde{I}|\le n'+d'/2 + d'/5 \le n'+d'$  and it has  $\le 2n'/3$ overlapping bits with $ z^{t}$. 
By \cref{prop:propertymainbasic}, the distance between $\tilde{I}$ and the zero codeword is $\ge d'$. 
So the distance between $I$ and the zero codeword is $\ge d' - d'/5 > d'/2$.
This is a contradiction since $I$ is in a match of $M$ and hence the distance between $I$ and the zero codeword is at most $d'/2$.
Thus $I'$ has overlaps with $\corrupted^t$ for $\le n'/3 - d'/10$ bits.
By the same analysis if $t' = t = t_0$, then $I'$ also need to have overlaps with $\corrupted^{t_0}$ for  $> 2n'/3 - d'/5 $ bits.
This is impossible.
The second possibility is that $b_1$ is zero. 
Notice that this means $b_1$ and $b_2$ are both zero.
$A(w)$ picks $b_2$ means $I$ inherits more bits from $b_2$.
As $|I| \ge n'-d'/2$, it inherits $\ge n'/2 - d'/4$ bits from $b_2$.
So $I$ has a size $\ge n'/2 - d'/4$ overlap with $\corrupted^{t_0}$.
Thus again $t' $ cannot be $t_0$.

As a result, $t \neq t'$ for any $i, i'$ from the two runs $A(w), A(w')$.

So the only possibility that distinct inputs can have the same output is that in the last rounds of their runs, their $I$ covers a same block which has more than $d'/4$ errors.
But in order to be an $I$ picked by $A$, the length of $I$ has to be at least $n'-d'/2$, since otherwise it cannot be matched to any block of $y$.
Hence there can be at most three distinct $I$s such that they cover a same block.
This shows our small claim.

The Claim follows by that there are at most $2T/d'$ unmatched blocks and there are at most $4T/d'$ blocks with at least $d'/4$ errors.
So $m_4 \leq 12T/d'$.



==> higherror2.tex <==
\section{Efficient Decoding of the Code in Section~\ref{sec:higherror}}\label{sec:herrordec}
We now give an efficient decoding algorithm for the code in Section~\ref{sec:higherror}. The algorithm is simple. Given any received string $y$, we consider the partition of $y$ into $n$ substrings $y_1, \cdots, y_n$ such that $y =y_1 \circ y_2 \circ \cdots \circ y_n$, where each $y_i$ can be the empty string. Now for each $y_i$, we find the closest codeword $x_i \in \Cin^i$ in insdel distance and record $\Delta_i=\ed(y_i, x_i)$. Finally we compute $\Delta=\sum_i \Delta_i$. Our goal is to minimize $\Delta$, and this can be done by using the following dynamic programming. 

We define a $n \times (N+1)$ matrix $f$ such that $\forall i \in [n], j \in [N] \cup \{0\}$, $f[i,j]$ records the optimal sum of insdel distances between a partition of $y_{[1:j]}$ into $i$ substrings and the concatenation of the first $i$ inner codewords. %Initially, we let $f[i,j] = 0$ if $i = 0 $ or $j = 0$. 

For any $0 \le p,  q \le N$, we define the function $g_i(y_{[p, q]})$ to be the insdel distance of the closest codeword $x_i \in \Cin^i$ to $y_{[p, q]}$. Note that the function $g_i$ can be computed in polynomial time by enumerating the $n$ codewords in $\Cin^i$ and computing the corresponding insdel distance to $y_{[p, q]}$. Now for $1\le i \le n$ and $0\le j \le N$, we can compute $f[i,j]$ as follows.

First, $\forall j \in  [N] \cup \{0\}$, let $f[1, j]=g_1(y_{[1, j]})$. Then, for $2\le i \le n$ and $ 0 \le j \le N$, we compute $f[i,j]$ using the following updating rule:

\[f[i,j] = 
\underset{0\le j' \le j}{\min} \; f[i-1, j'] + g_i(y_{[j'+1: j]}).
\]

Finally we return $f[n, N]$. To recover the inner codewords $\{x_i, i \in [n]\}$, during the dynamic programming we also maintain another $n \times (N+1)$ matrix $M$, such that $\forall i \in [n], j \in [N] \cup \{0\}$, $M[i, j]$ records two items: the right index of the previous substring (i.e., the optimal $j'$ in the updating rule), and the closest codeword $x_i \in \Cin^i$ to the substring $y_{[j'+1: j]}$. With these information one can trace back from $M[n, N]$ and recover all the inner codewords. 

After this, we use each $x_i$ to recover the corresponding symbol of the outer code at the $i$'th coordinate, and then run the list decoding algorithm from \cref{thm:listdecoding}. From the returned list, we exhaustively search for the codeword which has insdel distance less than $(1-6\gamma)N$ from the received string $y$.

We have the following lemma.

\begin{lemma}\label{lem:errorbound}
Assume the received string $y$ has at most $\alpha N$ insdel errors, then the above algorithm recovers at least $((1-2 \gamma)-\frac{\alpha}{1-2 \gamma}) n$ correct symbols in the outer codeword.
\end{lemma}

\begin{proof}
First note that there is a natural partition of $y$ according to the actual inner codewords. With this partition and let each $x_i$ be the corresponding correct inner codewords, one can see that the total insdel distance is at most $\alpha N$. Therefore, the optimal partition obtained by the dynamic programming must have $\Delta=\sum_i \Delta_i \leq \alpha N$.

Assume there are $\beta n$ symbols of the outer codeword that are recovered correctly after the algorithm. Let $z$ be the actual codeword transmitted without errors, and let $z_1, \cdots, z_n$ be the corresponding strings of $y_1, \cdots, y_n$ before errors, such that $z=z_1 \circ z_2 \circ \cdots \circ z_n$. 

Note that at most $2\gamma n$ of the $z_i$'s contains part of the codeword $0^{n'}$. Hence there are at least $(1-\beta-2 \gamma)n$ of the $z_i$'s that don't have the codeword $0^{n'}$ contributing to them, and are recovered to an incorrect inner codeword $x_i$ in the algorithm. For simplicity, let's pick exactly $(1-\beta-2 \gamma)n$ of such $z_i$'s.

We claim that any such $z_i$ and the incorrectly recovered inner codeword $x_i$ satisfy the conditions of Lemma~\ref{lem:property2}. To see this, notice that first of all, the codeword $0^{n'}$ does not contribute to $z_i$. Hence if $x_i=0$, then $x_i$ and $z_i$ satisfy the conditions of Lemma~\ref{lem:property2}. Otherwise, $x_i \neq 0$. If no codeword from $\Cin^i$ contributes to $z_i$, then by Property~\ref{prop:property1a}, $x_i$ and $z_i$ satisfy the conditions of Lemma~\ref{lem:property2}. Else, some codeword $x'_i \in \Cin^i$ contributes to $z_i$ and thus $x'_i$ is the correct inner codeword from $\Cin^i$. Since $x_i$ is recovered incorrectly, we must have $x_i \neq x'_i$, and again by Property~\ref{prop:property1a}, $x_i$ and $z_i$ satisfy the conditions of Lemma~\ref{lem:property2}. 

Therefore, let $B \subseteq [n]$ denote the index set of the $(1-\beta-2 \gamma)n$ of the $z_i$'s, and let $L=\sum_{i \in B} |z_i|$ be the total length of these $z_i$'s, by Lemma~\ref{lem:property2} we know that $\forall i \in B$, $\lcs(x_i, z_i) \leq 2\gamma(|x_i|+|z_i|)$. Thus

\[\sum_{i \in B} \ed(x_i, z_i) \geq \sum_{i \in B} (1-2\gamma)(|x_i|+|z_i|) \geq (1-2\gamma)((1-\beta-2 \gamma)N+L).\]

We now have two cases.

\begin{description}
\item [Case 1:] $L \geq (1-\beta-2 \gamma)N$. Then we have 
\[\sum_{i \in [n]} \ed(x_i, z_i) \geq \sum_{i \in B} \ed(x_i, z_i) \geq 2 (1-2\gamma)(1-\beta-2 \gamma)N.\]
\item [Case 2:] $L < (1-\beta-2 \gamma)N$. Then we have $\sum_{i \in [n] \setminus B} |z_i| = N-L$ and thus 
\[\sum_{i \in [n] \setminus B} \ed(x_i, z_i) \geq  \sum_{i \in [n] \setminus B} |z_i|- \sum_{i \in [n] \setminus B} |x_i| = N-L-(\beta+2 \gamma)N=(1-\beta-2 \gamma)N-L.\]

Thus
\begin{align*}
    \sum_{i \in [n]} \ed(x_i, z_i) &= \sum_{i \in B} \ed(x_i, z_i)+\sum_{i \in [n] \setminus B} \ed(x_i, z_i) \\ &\geq (1-2\gamma)((1-\beta-2 \gamma)N+L)+(1-\beta-2 \gamma)N-L \\ & > 2 (1-2\gamma)(1-\beta-2 \gamma)N.
\end{align*}
\end{description}
To conclude, we always have $\sum_{i \in [n]} \ed(x_i, z_i) \geq 2 (1-2\gamma)(1-\beta-2 \gamma)N.$ Now, since there are at most $\alpha N$ insdel errors, and the algorithm returns a matching such that $\Delta=\sum_i \Delta_i=\sum_i \ed(y_i, x_i) \leq \alpha N$, by triangle inequality we must have

\[2 (1-2\gamma)(1-\beta-2 \gamma)N \leq \sum_{i \in [n]} \ed(x_i, z_i) \leq \sum_{i \in [n]} \ed(x_i, y_i)+\alpha N \leq 2 \alpha N.\]

This gives 

\[\beta \geq (1-2 \gamma)-\frac{\alpha}{1-2 \gamma}.\]
\end{proof}

We can now prove the following theorem.

\begin{theorem}
For any constant $\gamma >0$, the code $\C$ can correctly decode from up to $1-6\sqrt{\gamma}$ fraction of insdel errors in polynomial time.
\end{theorem}

\begin{proof}
By \cref{lem:errorbound} and \cref{thm:listdecoding}, the list decoding algorithm of the outer code succeeds as long as 

\[(1-2 \gamma)-\frac{\alpha}{1-2 \gamma} \geq \sqrt{\gamma}.\]

At the same time, by \cref{lem:distance} the unique correct codeword can be found by examining the list of returned codewords as long as $\alpha \leq 1-6\gamma$.

One can check that when $\alpha \leq 1-6\sqrt{\gamma}$, both conditions are satisfied.
\end{proof}

By setting $\gamma=\frac{\eps^2}{36}$, this immediately gives the following corollary.

\begin{corollary}
For any constant $\eps >0$, there is a linear code $\C$ with rate $\Omega(\eps^4)$ and alphabet size $\poly(1/\eps)$, that can be encoded in polynomial time and decoded from up to $1-\eps$ fraction of insdel errors in polynomial time.
\end{corollary}
